A Literature Based Approach to Define the Scope of Biomedical Ontologies: A Case Study on a Rehabilitation Therapy Ontology

In this article, we investigate our early attempts at building an ontology describing rehabilitation therapies following brain injury. These therapies are wide-ranging, involving interventions of many different kinds. As a result, these therapies are hard to describe. As well as restricting actual practice, this is also a major impediment to evidence-based medicine as it is hard to meaningfully compare two treatment plans. Ontology development requires significant effort from both ontologists and domain experts. Knowledge elicited from domain experts forms the scope of the ontology. The process of knowledge elicitation is expensive, consumes experts' time and might have biases depending on the selection of the experts. Various methodologies and techniques exist for enabling this knowledge elicitation, including community groups and open development practices. A related problem is that of defining scope. By defining the scope, we can decide whether a concept (i.e. term) should be represented in the ontology. This is the opposite of knowledge elicitation, in the sense that it defines what should not be in the ontology. This can be addressed by pre-defining a set of competency questions. These approaches are, however, expensive and time-consuming. Here, we describe our work toward an alternative approach, bootstrapping the ontology from an initially small corpus of literature that will define the scope of the ontology, expanding this to a set covering the domain, then using information extraction to define an initial terminology to provide the basis and the competencies for the ontology. Here, we discuss four approaches to building a suitable corpus that is both sufficiently covering and precise.

==> temp.tex <==


\subsection{PubMed's similar articles functionality (PMSA)}
\label{PMSA}

PubMed's similar articles functionality (PMSA) is based on text
similarity. Currently, it only supports retrieving citations similar
to one user selected citation. It is not directly applicable for
retrieving citations similar to multiple user selected citations,
i.e. seed set of citations, as can be seen in figure~\ref{fig:pmsa}
. Different approaches can be used to extend
PMSA~\citep{pitigala2014extending} to retrieve citations similar to a
seed set of citations.  The basic approach is to apply PMSA on each
citation in the seed set, and combine all the retrieved
citations. However, the basic approach is usually not good in
capturing the concept expressed through the multiple
citations~\citep{pitigala2014extending}.

\begin{figure}[htpb]
\centering
\includegraphics[width=\linewidth]{pmsa.jpg}
\caption{PubMed's similar articles (PMSA) supports retrieving articles
  similar to one citation only. It can only retrieve articles similar
  to citation A or Hcc, each at time, but not articles similar to both
  of them}
\label{fig:pmsa}
\end{figure}
xo
